What Challenges Do Developers Face About Checked-in Secrets in Software Artifacts?

Throughout 2021, GitGuardian's monitoring of public GitHub repositories revealed a two-fold increase in the number of secrets (database credentials, API keys, and other credentials) exposed compared to 2020, accumulating more than six million secrets. To our knowledge, the challenges developers face to avoid checked-in secrets are not yet characterized. The goal of our paper is to aid researchers and tool developers in understanding and prioritizing opportunities for future research and tool automation for mitigating checked-in secrets through an empirical investigation of challenges and solutions related to checked-in secrets. We extract 779 questions related to checked-in secrets on Stack Exchange and apply qualitative analysis to determine the challenges and the solutions posed by others for each of the challenges. We identify 27 challenges and 13 solutions. The four most common challenges, in ranked order, are: (i) store/version of secrets during deployment; (ii) store/version of secrets in source code; (iii) ignore/hide of secrets in source code; and (iv) sanitize VCS history. The three most common solutions, in ranked order, are: (i) move secrets out of source code/version control and use template config file; (ii) secret management in deployment; and (iii) use local environment variables. Our findings indicate that the same solution has been mentioned to mitigate multiple challenges. However, our findings also identify an increasing trend in questions lacking accepted solutions substantiating the need for future research and tool automation on managing secrets.

==> Tables/AnswerCodebook.tex <==
\newcolumntype{s}{>{\hsize=0.03\hsize}X}
\newcolumntype{b}{>{\hsize=0.6\hsize} X}
\newcolumntype{m}{>{\hsize=0.4\hsize}X}
\begin{table}
\centering
\small
\caption{Codebook for Answers}
\label{answer-codebook}
%\scriptsize
\footnotesize
%\tiny
\begin{tabularx}{\columnwidth} {|m|b|}
\hline
\multicolumn{1}{|c|}{\textbf{Answer Category}} & \multicolumn{1}{l|}{\textbf{Answer Sub-category}} \\ \hline \hline
Revokation and Rotation & None \\ \hline
\multirow{1}{*}{Rewrite VCS History} & Use of git-filter-branch, Use of git-filter-repo, BFG Repo Cleaner, Use of Git Rebase, Git Reset --hard \\ \hline
 
\multirow{1}{*}{VCS Feature} & Git Flags (Git attribute custom driver, pre-commit and post-update hook), Git Flags (--skip-worktree, update-index --assume-unchanged) \\ \hline
 
VCS Scan Tool & Gitrob, TruffleHog \\ \hline
Add Files to the Staging Area Explicitly & Avoid git add -A \\ \hline

\multirow{1}{*}{Ignore Sensitive File} & Secrets in Config. File, Secrets in Non-Config. File \\ \hline

Store Encrypted or Obfuscated Secrets & Base64 Encoding, Master Password, Split into Multi Parts, AES encryption, MD5 Encryption, Hashing Secrets \\ \hline
 

Secret Management in Deployment & Deployment Tools (TeamCity, AWS Codedeploy, Capistrano, Github Actions, Travis CI), Configuration Management Systems (Ansible-Vault), Deployment Variables (Heroku Config Vars, Github Secret, CircleCI variable, Google Cloud VM Metadata), Shared Folder (Capistrano Shared Directory), Keep dot file out of root directory (.git , .git-credentials, .hg), Mask Secrets in log (Github actions add-mask) \\ \hline



External Secret Management Service & HashiCorp vault, Square's Keywhiz, Pinterest's Knox  \\ \hline

Use Local Environment Variables & OS level (dotenv library), Platform level (Java Properties) \\ \hline

Restrict API access and permissions & None \\ \hline

No Rely on Code Review  & None \\ \hline

Remove Original Config. File  & None \\ \hline

Use Template Config. File & Place dummy secrets in config. file \\ \hline

Move Secrets to Config. File & None \\ \hline

Move Secrets out of Source Code and Version Control & None \\ \hline
\multirow{1}{*}{Load Externally} & Load from S3, Place secrets in external file/folder \\ \hline

Secondary Private Repository & None \\ \hline
Non Exploitable & None \\ \hline
Exploitable & None \\ \hline
Server Side Implementation & None \\ \hline
Coding Syntax Fix & None \\ \hline 

Others & Add security.md file, Disable forking \\ \hline 
     
\end{tabularx}
\end{table}

==> Tables/CombinedUpdatedMappingsTables.tex <==
\begin{table}[]
\footnotesize
%\centering
\caption{Configuration File and Secrets Mappings Table}
\label{my-label}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{ |p{2.5cm}|p{2cm}|p{10cm}| }
\hline
\textbf{Domain} & \textbf{Question Category} & \textbf{Answers} \\ \hline %\cline{3-7} 
  %& & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
  
\multirow{5}{*}{Configuration File} & Store/Version & Ignore Sensitive File, Store Encrypted/Obfuscated Secrets (GPG, Bouncy Castle Libs Encryption), Secret Management in Deployment (Configuration Transformation, Deployment Variables: Heroku Configuration Variables, Shared Folder, Create Configuration File in Deployment Server), External Secret Management Service (AWS parameter store, git-secrets, Travis CI, Vault), Use Environment Variables, Remove Original Configuration File, Use a Template Configuration file (commit a template configuration file with dummy secrets), Move Secrets out of Source Code/Version Control, Secondary Private Repository, Non-Exploitable \\ \cline{2-3} 
 & Ignore/Hide &  Ignore Sensitive File (Configuration File, .env file), Add Files to the Staging Area Explicitly, Store Encrypted/Obfuscated Secrets (Encrypted: Protected Configuration), Secret Management in Deployment (Run time configuration loading), Use Environment Variables, Remove Original Configuration File, Use Environment Variables, Use a Template Configuration file (commit a template configuration file with dummy secrets), Move Secrets out of Source Code/Version Control, Load Externally\\ \cline{2-3}
 & Distribute &  Ignore Sensitive File, Use Template Configuration File, Move Secrets out of Source Code/Version Control\\ \cline{2-3}
 & Exploitability &  Use Environment Variables, External Secret Management Service, Move Secrets out of Source Code, Non-Exploitable\\ \cline{2-3}
 & Accessibility &  Secret Management in Deployment (Configuration Transformation), Syntax Error Fix\\ \hline
 
 \multirow{5}{*}{Secrets} & Store/Version & Revokation and Rotation (Rotate Compromised Credential), Ignore Sensitive File (Configuration File, Web Configuration File, Secrets in Non-Configuration File), Store Encrypted/Obfuscated Secrets  (AES Encryption, AES128-CBC Encryption, Base64 Encoding, DES Encryption, Encrypt Sensitive Sections, Master Key for Encrypted Secrets, Master Password, MD5 Encryption, RSA Encryption, Split into Multi Parts), Secret Management in Deployment (Create Configuration file in Deployment Server, Deployment Tools, Deployment Variables (\textbf{Repeat?}), Deployment Variables -> Heroku Configuration Variables, Configuration Transformation (web configuration)), External Secret Management Service (Azure key Vault, Cloud KMS, Hashicorp/Vault, square keyWhiz), Use Environment Variables (OS level -> Using dotenv library, Platform level: Java Properties), Restrict API access and permissions, Use a Template Configuration file (commit a template config file with dummy secrets), Use Template Non-Config file (commit a template non- config file with dummy secrets), \textbf{Keep Secrets out of Configuration File??}, Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Load Externally, Server Side Implementation (Retrieve secret key from server) \\ \cline{2-3} 
 
 & Ignore/Hide &  Revokation and Rotation (Rotate Compromised Credential), Rewrite VCS History (Use Git Filter Branch, BFG Repo Cleaner, Git Filter Repo), Ignore Sensitive File (Configuration File, Secrets in Non-Configuration File), VCS Feature (VCS Hooks: (Git attribute custom driver, pre-commit and post-commit hooks, Git hooks)), Store Encrypted/Obfuscated Secrets (Base 64 Encoding, Encrypt sections of web. config file, Data Protection API (DPAPI), Net 2.0 Protected Data Class), Secret Management in Deployment(Configuration Transformation, Deployment Variables - (Heroku Config Vars, Github Secret), Shared Folder: Capistrano), External Secret Management Service (Secure Storage by Xlab, Hashicorp Vault), Use Environment Variables, Use Template Configuration File (commit a template non- config file with dummy secrets), Use Non- Template Configuration file (commit a non-template configuration file with dummy secrets), Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Secondary Private Repository, Server Side Implementation, \textbf{improper set up??}\\ \cline{2-3}
 
 & Distribute &  Ignore Sensitive File (Secrets in Non-Configuration File), Secret Management in Deployment (Deployment Tools AWS),  Use Template Config file (secrets file), Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Load Externally\\ \cline{2-3}
 
 & Exploitability &  Revokation and Rotation (Rotate Compromised Credential), Rewrite VCS History (Use of Git Filter Branch), Ignore Sensitive File, Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Non Exploitable, Exploitable
\\ \cline{2-3}
 
 & Restriction &  Restrict API access and permissions\\ \hline
 
%\multirow{4}{*}{Secrets} & Answer 0 &  &  &  &  & \\ \cline{2-7} 
% & Answer 1 & &  &  &  &  \\ \cline{2-7} 
% & Answer 2 &  &  &  &  &  \\ \cline{2-7} 
% & Answer 3 &  &  &  &  &  \\ \hline
%\multirow{4}{*}{Client Side} & Answer 0 &  &  &  &  & \\ \cline{2-7} 
% & Answer 1 & &  &  &  &  \\ \cline{2-7} 
% & Answer 2 &  &  &  &  &  \\ \cline{2-7} 
% & Answer 3 &  &  &  &  &  \\ \hline
 %\multicolumn{7}{|c|}{} \\ \hline 
 
\end{tabular}
\end{table}


\begin{table}[]
\footnotesize
%\centering
\caption{Client Side Application, VCS Feature Table, Pre Open Source, Secureness, External Secret Management, Others}
\label{my-label}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{ |p{3 cm}|p{2cm}|p{9cm}| }
\hline
\textbf{Domain} & \textbf{Question Category} & \textbf{Answers} \\ \hline %\cline{3-7} 
  %& & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
  
\multirow{3}{*}{Client Side Application} & Store & Revokation and Rotation (Rotate Compromised Credential), Store Encrypted/Obfuscated Secrets (Hashing Secrets, HTML Resource 5 Encryption, Obfuscate Secrets, PKCE), Use Environment Variables, Move Secrets out of Source Code/Version Control, Non Exploitable, Server Side Implementation
\\ \cline{2-3} 

 & Hide &   Revokation and Rotation (Short lived secrets), Use Environment Variables, Move Secrets out of Source Code/Version Control, Server-Side Implementation \\ \cline{2-3}
 
 & Exploitability &   Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Non-Exploitable, Exploitable\\ \hline
 
 
 \multirow{4}{*}{VCS Feature} & History Sanitize & Revokation and Rotation (Rotate Compromised Credential), Rewrite VCS History (Use of Git Filter Branch, Git Filter Repo, BFG Repo Cleaner, Git Reset –hard, Git Rebase), Ignore Sensitive File (Secrets in Non-Configuration File), VCS Scan Tool (Truffle Hog, Gitrob), Add Files to the Staging Area Explicitly, Use Template Configuration  file, Move Secrets to Configuration File, Secondary Private Repository
 \\ \cline{2-3} 
 
 & Line Level Security &  Ignore Sensitive File (Secrets in Non-configuration File, Configuration File), VCS Feature (Git Hooks: Pre-commit and post-update hook, Git attribute custom driver), Add Files to the Staging Area Explicitly, Store Encrypted/Obfuscated Secrets (Rails Secrets), Use Environment Variables Use a Template Configuration file (commit a template configuration file with dummy secrets), Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Secondary Private Repository
 \\ \cline{2-3}
 
 & Encrypt File &  VCS Feature (VCS Hook: pre-commit and post-commit)\\ \cline{2-3}
 
 & Ignore Already Committed &  Rewrite VCS History, Ignore Sensitive File, VCS Feature (Git Flag : git --skip-worktree, use of git update-index -- assume unchanged), Use Environment Variable, Use Template Config file (commit a template config file with dummy secrets), Remove Original Configuration File, Use Template Config File

\\ \hline
 
 
Pre Open Source & Crosscheck & Rewrite VCS History (Use of Git Filter Branch, Git Filter Repo, BFG Repo Cleaner), Ignore Sensitive File  (Configuration File, Secrets in Non-Configuration File), Store Encrypted/Obfuscated Secrets (Travis CI-Integration Encryption), Secret Management in Deployment (Deployment Variables -> Heroku Config Vars, Mask Secrets in log), External Secret Management Service (cloud KMS), Use Environment Variables, Use a Template Configuration file (commit a template configuration file with dummy secrets), Use Template non-Configuration file (commit a template non- configuration file with dummy secrets), Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control, Load Externally, Secondary Private Repository, Non-Exploitable, Server-Side Implementation
\\ \hline 

\multirow{2}{*}{Secureness} & Private Repository & External Secret Management Service (Vault Instance), Use Template Config file, Move Secrets out of Source Code/Version Control, Load Externally, Non-Exploitable, Exploitable
\\ \cline{2-3}

& Unpushed Branch & Ignore Sensitive File (Configuration File), Move Secrets to Configuration File, Move Secrets out of Source Code/Version Control
\\ \hline

External Secret Management & Setup & Load Externally
\\ \hline

\multirow{2}{*}{Others} & Importance & No Accepted Answer
\\ \cline{2-3}

& Decision & Revokation and Rotation (Rotate Compromised Credential)
\\ \hline



 %& Restriction &  Restrict API access and permissions\\ \hline
 
%\multirow{4}{*}{Secrets} & Answer 0 &  &  &  &  & \\ \cline{2-7} 
% & Answer 1 & &  &  &  &  \\ \cline{2-7} 
% & Answer 2 &  &  &  &  &  \\ \cline{2-7} 
% & Answer 3 &  &  &  &  &  \\ \hline
%\multirow{4}{*}{Client Side} & Answer 0 &  &  &  &  & \\ \cline{2-7} 
% & Answer 1 & &  &  &  &  \\ \cline{2-7} 
% & Answer 2 &  &  &  &  &  \\ \cline{2-7} 
% & Answer 3 &  &  &  &  &  \\ \hline
 %\multicolumn{7}{|c|}{} \\ \hline 
 
\end{tabular}
\end{table}


\begin{table}[]
\footnotesize
%\centering
\caption{Deployment Mappings Table}
\label{my-label}
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{ |p{2.5cm}|p{2cm}|p{10cm}| }
\hline
\textbf{Domain} & \textbf{Question Category} & \textbf{Answers} \\ \hline %\cline{3-7} 
  %& & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
  
\multirow{4}{*}{Deployment} & Store/Version & Ignore Sensitive File (Configuration File, Secrets in Non-Configuration File), VCS Feature (Git Hooks: Git attribute custom driver), Store Encrypted/Obfuscated Secrets (RSA, Split into Multi Parts, ASP.NET Registration Tool Encryption, Rails encryption secrets, KeyPass, AES256 encryption, R8, JNI/IDK), Secret Management in Deployment (Create configuration file in Deployment Server, Configuration Transformation (Encrypt sectiong of configuration file, SlowCheetah, ReplaceTokens), web configuration transformation, Deployment Tools (Circle CI), Deployment Variables: (Heroku Configuration Variables, Appharbor Configuration Variables, Google Cloud Datastore, Azure portal app settings, Azure Portal, Elastic Beanstalk Environment Variables, GAE settings?), Configuration Management System - puppet, chef, Ansible-Vault, Azure, Spring Cloud Config), External Secret Management Service (Hashicorp Vault, Azure Key Vault, AWS Secrets Manager, Conjur, okta), Use Environment Variables (Non-specific, OS level -> Using dotenv library), Restrict API access and permissions, Use a Template Configuration file (commit a template configuration file with dummy secrets, second.env file??), Move Secrets out of Source Code/Version Control, Load Externally (S3), Secondary Private Repository, Server-Side Implementation, \textbf{Keep Secrets out of Configuration File?} \\ \cline{2-3} 

 & Ignore/Hide &  Ignore Sensitive File (Secrets in Non-Configuration File), Store Encrypted/Obfuscated Secrets (Mask Passwords Plugin), Secret Management in Deployment (Deployment Variables : Heroku Config Vars, Keep dot file out of root directory), External Secret Management Service (Azure key Vault), Use Environment Variables
, Use Non-Template Configuration file (commit a non-template configuration file with dummy secrets), \textbf{Store encrypted config file locally??, use template config file in repo?}
\\ \cline{2-3}
 
 & Improper Configuration &  Ignore Sensitive File (Configuration File, Secrets in Configuration File), Secret Management in Deployment (Deployment Tools: Github Actions, Deployment Variables -> Heroku Config Vars), External Secret Management Service (AWS Secret Manager), Use Environment Variables, Use Template Config file (commit a template config file with dummy secrets), Use Template Non-Config file (commit a template non-config file with dummy secrets), Move Secrets out of Source Code/Version Control,
\\ \cline{2-3}
 & Dot-File &  Secret Management in Deployment (Keep dot file out of root directory), Exploitable
\\ \hline
 %& Accessibility &  Secret Management in Deployment (Configuration Transformation), Syntax Error Fix\\ \hline
 
 \end{tabular}
\end{table}

==> Tables/FinalAnswerMappingsTables.tex <==
\newcolumntype{s}{>{\hsize=0.03\hsize}X}
\newcolumntype{b}{>{\hsize=0.75\hsize} X}
\newcolumntype{m}{>{\hsize=0.15\hsize}X}
\begin{table*}
\centering
\caption{Answer to RQ2. The mapping of answers to each question category}
\label{question-answer-mapping}
\footnotesize
%\tiny
\begin{tabularx}{\textwidth} {|s|m|b|}
\hline
\multicolumn{1}{|c|}{\textbf{Domain}} & \multicolumn{1}{l|}{\textbf{Question Category}} & \multicolumn{1}{c|}{\textbf{Answer Category}} \\ \hline \hline
\multirow{5}{*}{Secrets}
 & Q1: Store/Version & Revokation and Rotation, Move Secrets out of Source Code/Version Control and Use Template Config File, Secret Management in Deployment (Deployment Variables, Config Transformations), Use of External Secret Management Service (HashiCorp Vault and Azure key Vault), Use Local Environment Variables, Restrict API Access and Permissions, Load Externally and Use Secondary Private Repository, Server-Side Implementation \\ \cline{2-3}
 
 & Q2: Ignore/Hide & Revokation and Rotation, Rewrite VCS History (Use git-filter-branch, git-filter-repo and BFG repo cleaner), Move Secrets out of Source Code/Version Control and Use Template Config File, VCS Feature (Git Hooks: Git attribute custom driver, pre-commit and post-commit hooks), Store Encrypted/Obfuscated Secrets, Secret Management in Deployment (Deployment Variables, Config Transformations, Shared Directory), Use of External Secret Management Service (HashiCorp Vault and Azure key Vault), Use Local Environment Variables, Load Externally and Use Secondary Private Repository, Server-Side Implementation\\ \cline{2-3}
 
  & Q3: Exploitability & Revokation and Rotation, Rewrite VCS History (Use of git-filter-branch), Move Secrets out of Source Code/Version Control and Use Template Config File \\ \cline{2-3}
 
 & Q4: Distribute & Move Secrets out of Source Code/Version Control and Use Template Config File, Secret Management in Deployment, Load Externally and Use Secondary Private Repository \\ \cline{2-3}

 
 & Q5: Restriction & Restrict API Access and Permissions \\ \hline
 
   \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}Deploy-\\ment\end{tabular}} 
 & Q6: Store/Version & Move Secrets out of Source Code/Version Control and Use Template Config File, VCS Feature (Git attribute custom driver), Store Encrypted/Obfuscated Secrets, Secret Management in Deployment (Config Transformation, Deployment Variables, Configuration Management Systems (Puppet, Ansible-Vault)), Use of External Secret Management Service (HashiCorp Vault, Azure Key Vault), Use Local Environment Variables, Restrict API Access and Permissions, Load Externally (S3) and Use Secondary Private Repository, Server-Side Implementation \\ \cline{2-3} 
 
  & Q7: Improper Configuration & Move Secrets out of Source Code/Version Control and Use Template Config File, Secret Management in Deployment (Deployment Tools: GitHub Actions, Deployment Variables), External Secret Management Service (AWS Secret Manager), Use Local Environment Variables
\\ \cline{2-3}
 
 & Q8: Ignore/Hide & Move Secrets out of Source Code/Version Control and Use Template Config File, Store Encrypted/Obfuscated Secrets (Mask Passwords Plugin), Secret Management in Deployment (Deployment Variables, Keep dot file out of root directory), Use of External Secret Management Service (Azure key Vault), Use Local Environment Variables
\\ \cline{2-3}

 
 & Q9: Dot File  & Secret Management in Deployment (Keep dot file out of root directory) \\ \hline
 
 \multirow{4}{*} {\begin{tabular}[l]{@{}l@{}}VCS \\Feature\end{tabular}} 
  & Q10: History Sanitize & Revokation and Rotation, Rewrite VCS History (Use git-filter-branch, git-filter-repo, BFG repo cleaner, git reset --hard, git rebase), Move Secrets out of Source Code/Version Control and Use Template Config File, VCS Scan Tools (Truffle Hog, Gitrob), Load Externally and Use Secondary Private Repository
 \\ \cline{2-3} 
 
  & Q11: Ignore Already Committed  & Rewrite VCS History, Move Secrets out of Source Code/Version Control and Use Template Config File, VCS Feature (Git Flags: git --skip-worktree, git update-index --assume-unchanged), Use Local Environment Variable \\ \cline{2-3}
  
  & Q12: Line Level Security & Move Secrets out of Source Code/Version Control and Use Template Config File, VCS Feature (Git Hooks: Git attribute custom driver, pre-commit and post-update hook), Add Files to the Staging Area Explicitly, Store Encrypted/Obfuscated Secrets (Rails Secrets), Use Local Environment Variables, Load Externally and Use Secondary Private Repository
 \\ \cline{2-3}
  
   & Q13: Encrypt File & VCS Feature (Git Hooks: pre-commit and post-commit) \\ \hline
 
 \multirow{5}{*} {\begin{tabular}[l]{@{}l@{}}Configur-\\ ation File\end{tabular}}   
 & Q14: Store/Version & Move Secrets out of Source Code/Version Control and Use Template Config File, Store Encrypted/Obfuscated Secrets, Secret Management in Deployment (Deployment Variables, Config Transformations, Shared Directory), Use of External Secret Management Service, Use Local Environment Variables, Load Externally and Use Secondary Private Repository \\ \cline{2-3}  
 
  & Q15: Ignore/Hide & Move Secrets out of Source Code/Version Control and Use Template Config File, Add Files to the Staging Area Explicitly, Store Encrypted/Obfuscated Secrets, Secret Management in Deployment, Use Local Environment Variables, Load Externally and Use Secondary Private Repository\\ \cline{2-3}
  
 & Q16: Distribute &  Move Secrets out of Source Code/Version Control and Use Template Config File \\ \cline{2-3}
    
    & Q17: Exploitability & Use Local Environment Variables, Use of External Secret Management Service, Move Secrets out of Source Code/Version Control and Use Template Config File \\ \cline{2-3}
    
     & Q18: Accessibility & Secret Management in Deployment (Config Transformation) \\ \hline
     
      \multirow{1}{*}{\begin{tabular}[l]{@{}l@{}}Pre-open\\ Source\end{tabular}} 
 & Q19: Cross-check & Rewrite VCS History (Use of git-filter-branch, git-filter-repo, BFG repo cleaner), Move Secrets out of Source Code/Version Control and Use Template Config File, Store Encrypted/Obfuscated Secrets, Secret Management in Deployment (Deployment Variables, Mask Secrets in log), Use of External Secret Management Service (Cloud KMS), Use Local Environment Variables, Load Externally and Use Secondary Private Repository, Server-Side Implementation \\ \hline
     
  \multirow{3}{*} {\begin{tabular}[l]{@{}l@{}}Client- \\Side\\Applicat-\\ion\end{tabular}} 
  & Q20: Store & Revokation and Rotation, Store Encrypted/Obfuscated Secrets, Use Local Environment Variables, Move Secrets out of Source Code/Version Control and Use Template Config File, Server-Side Implementation
\\ \cline{2-3} 
  
  & Q21: Hide & Revokation and Rotation, Use Local Environment Variables, Move Secrets out of Source Code/Version Control and Use Template Config File, Server-Side Implementation \\ \cline{2-3}
  
  & Q22: Exploitability  & Move Secrets out of Source Code/Version Control and Use Template Config File \\ \hline
  
    \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Secure-\\ness\end{tabular}} 
 & Q23: Private Repository & Use of External Secret Management Service, Move Secrets out of Source Code/Version Control and Use Template Config File, Load Externally and Use Secondary Private Repository
\\ \cline{2-3}
 
  & Q24: Unpushed Branch & Move Secrets out of Source Code/Version Control and Use Template Config File \\ \hline
 
  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Ext. Sec. \\ Mng.. \end{tabular}} 
 & Q25: Setup  & Load Externally and Use Secondary Private Repository \\
 &   & \\\hline
  
  \multirow{2}{*}{Others} 
 & Q26: Importance & No Accepted Answer \\ \cline{2-3}
 
  & Q27: Decision  & Revokation and Rotation\\ 
  \hline
     
\end{tabularx}
\end{table*}

==> Tables/Part1Mappings.tex <==
\begin{table}[]
\tiny
\centering
\caption{Mappings Table}
\label{my-label}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Question Category}} & \multirow{2}{*}{\textbf{Answer Category}} & \multicolumn{5}{l|}{Sub Categories} \\ \cline{3-7} 
  & & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
  
\multirow{4}{*}{Config File} & Rewrite VCS History &  &  & X &  & \\ \cline{2-7} 

 & Ignore Sensitive File & X & X & X &  & \\ \cline{2-7} 
 & VCS Feature &  &  & X &  &\\ \cline{2-7} 
  & Add Files to the Staging Area Explicitly &  &  &  X &  &\\ \cline{2-7} 
   & Store Encrypted/Obfuscated Secrets &X  &  & X &  &\\ \cline{2-7} 
   & Secrets Management in Deployment &  &  &  &  &\\ \cline{2-7} 
 & Config Transformation &  X&  &  & X  &\\ \cline{2-7}
 & Deployment Variables &  X&  &  &   &\\ \cline{2-7}
 & Shared Folder &  X&  &  &   &\\ \cline{2-7}
 & Create config file in Deployment  Server &  X&  &  &   &\\ \cline{2-7}
 & External Secret Management Service & X &  &  &  & X\\ \cline{2-7} 
  & Use Environment Variables & X &  & X &  & X\\ \cline{2-7} 
  &  Remove Original Config File & X &  & X &  &\\ \cline{2-7} 
   &  Use Template File & X & X & X &  &\\ \cline{2-7} 
    & Move Secrets out of S.C/V.S. & X &  & X &  & X\\ \cline{2-7} 
    &  Load Externally &  &  & X &  &\\ \cline{2-7}
&      Secondary Private Repository & X &  &  &  &\\ \cline{2-7}
& Non Exploitable & X &  &  &  & X\\ \hline 
 %& Answer 3 &  &  &  &  &  \\ \hline
\multirow{4}{*}{Secrets} & Revokation and Rotation & X &  &X  &  &X \\ \cline{2-7} 
   
& Rewrite VCS History &  &  & X &  & X \\ \cline{2-7} 

 & Ignore Sensitive File & X &  & X &  & \\ \cline{2-7} 
 & VCS Feature &  &  & X &  &\\ \cline{2-7} 
 &  Store Encrypted/Obfuscated Secrets &X  &  & X &  &\\ \cline{2-7} 
& Deployment Tools &  X&  &  &   &\\ \cline{2-7} 
& Config Transformation &  X&  & X &   &\\ \cline{2-7}
& Deployment Variables &  X&  & X &   &\\ \cline{2-7}
& Shared Folder &  &  & X &   &\\ \cline{2-7}
& Create config file in Deployment Server & X &  &  &   &\\ \cline{2-7}
&  External Secret Management Service & X &  & X  &  & \\ \cline{2-7} 
 &  Use Environment Variables & X &  & X &  & \\ \cline{2-7} 
  & Restrict API access and permissions & X &  &  &  &\\ \cline{2-7}
  &   Use Template Config/Non-Config file & X &  & X &  &\\ \cline{2-7} 
  &   Move Secrets to Configuration File & X &  & X &  & \\ \cline{2-7}
  &   Move Secrets out of Source Code/Version Control & X &  & X &  & X\\ \cline{2-7} 
  &    Load Externally & X & X & X &  &\\ \cline{2-7}
  &    Secondary Private Repository &  &  & X &  &\\ \cline{2-7} 
  &    Non Exploitable &  &  &  &  & X\\ \cline{2-7} 
  &    Exploitable &  &  &  &  & X\\ \cline{2-7} 
  &    Server Side Implementation & X &  & X &  & \\ \hline
  
  
\multirow{4}{*}{Client Side} & Revokation and Rotation &  &  &  &  & \\ \cline{2-7} 

& Store Encrypted/Obfuscated Secrets &X  &  &  &  &\\ \cline{2-7} 
 &  Use Environment Variables & X &  & X &  & \\ \cline{2-7} 

 &    Move Secrets to Configuration File &  &  &  &  & X\\ \cline{2-7}
 &    Move Secrets out of Source Code/Version Control & X &  &  &  & X\\ \cline{2-7} 
 &     Non Exploitable & X &  &  &  & X\\ \cline{2-7}
 &     Exploitable &  &  &  &  & X\\ \cline{2-7}
 &     Server Side Implementation & X &  & X &  & \\ \hline
 
 \multirow{2}{*}{\textbf{Question Category}} & \multirow{2}{*}{\textbf{Answer Category}} & \multicolumn{5}{l|}{Sub Categories} \\ \cline{3-7} 
  & & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
 
 
\multirow{4}{*}{Deployment} & Ignore Sensitive File &  &  &  &  & \\ \cline{2-7} 
& VCS Feature &  &  & X &  &\\ \cline{2-7} 
 &  Store Encrypted/Obfuscated Secrets &X  &  & X &  &\\ \cline{2-7} 
& Deployment Tools  &  X& X &  & X  &\\ \cline{2-7} 
& Configuration Management System  &  X&  &  &   &\\ \cline{2-7}
& Config Transformation
  &  X&  &  &   &\\ \cline{2-7}
&  Deployment Variables  &  X&  & X & X  &\\ \cline{2-7}
&  Keep dot file out of root directory &  &  & X &   &X\\ \cline{2-7}
&  Create config file in Deployment Server & X &  &  &   &\\ \cline{2-7}
&  External Secret Management Service & X &  & X  & X & \\ \cline{2-7} 
&   Use Environment Variables & X &  & X & X & \\ \cline{2-7} 
&   Restrict API access and permissions & X & X & X & X &\\ \cline{2-7}
&     Use Template Config/Non-Config file & X & X & X & X  &\\ \cline{2-7} 
&     Move Secrets out of Source Code/Version Control & X &  X&  & X & \\ \cline{2-7} 
&      Load Externally & X &  & X &  &\\ \cline{2-7}
&      Secondary Private Repository & X &  &  &  &\\ \cline{2-7} 
&      Exploitable &  &  &  &  & X\\ \cline{2-7} 
&      Server Side Implementation & X &  &  &  & \\ \hline 
 
 
  \multirow{2}{*}{\textbf{Question Category}} & \multirow{2}{*}{\textbf{Answer Category}} & \multicolumn{5}{l|}{Sub Categories} \\ \cline{3-7} 
  & & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
 
 
\multirow{4}{*}{Version Control Feature} & Revokation and Rotation &  &  &  &  & \\ \cline{2-7} 
 
& Rewrite VCS History & X &  &  &  &\\ \cline{2-7}
 &  Ignore Sensitive File & X & X &  &  &\\ \cline{2-7}
 &  VCS Feature &  &  & X &  &\\ \cline{2-7}
 &   VCS Scan Tool & X &  &  &  &\\ \cline{2-7} 
 &  Add Files to the Staging Area Explicitly & X & X &  &  &\\ \cline{2-7} 
 &  Store Encrypted/Obfuscated Secrets &  & X &  &  &\\ \cline{2-7} 
 &  Use Environment Variables &  & X &  &  & \\ \cline{2-7} 
 &  Use Template Config/Non-Config File &  & X &  &  & \\ \cline{2-7} 

  &   Move Secrets to Configuration File &  & X &  &  & \\ \cline{2-7}
   &  Move Secrets out of Source Code/Version Control &  & X  &  &  & \\ \cline{2-7} 
&     Secondary Private Repository & X & X &  &  & \\ \hline 
 
 
  \multirow{2}{*}{\textbf{Question Category}} & \multirow{2}{*}{\textbf{Answer Category}} & \multicolumn{5}{l|}{Sub Categories} \\ \cline{3-7} 
  & & Store/Version & Distribute & Ignore/Hide & Accessibility & Exploitability \\ \hline
 
 
\multirow{4}{*}{Pre Open Source} & Rewrite VCS History &  &  &  &  & \\ \cline{2-7} 
 
 
& Ignore Sensitive File & X &  &  &  & \\ \cline{2-7}
& Store Encrypted/Obfuscated Secrets & X &  &  &  & \\ \cline{2-7}
& Deployment Variables & X &  &  &  & \\ \cline{2-7}
& Mask Secrets in log & X &  &  &  & \\ \cline{2-7}

 &  External Secret Management Service & X &  &  &  & \\ \cline{2-7}
 &  Use Environment Variables & X &  &  &  & \\ \cline{2-7} 
 &  Use Template Config/Non-Config File & X &  &  &  & \\ \cline{2-7} 
 &  Move Secrets to Configuration File & X &  &  &  & \\ \cline{2-7} 
 &    Move Secrets out of Source Code/Version Control & X &  &  &  & \\ \cline{2-7} 
 &    Load Externally & X &  &  &  & \\ \cline{2-7} 
 &    Secondary Private Repository & X &  &  &  & \\ \cline{2-7}
 &     Non Exploitable & X &  &  &  & \\ \cline{2-7}
 &     Exploitable & X &  &  &  & \\ \cline{2-7}
 &     Server Side Implementation & X &  &  &  & \\ \hline
 
 
\end{tabular}
\end{table}

==> Tables/QuestionCodebook.tex <==
\begin{table}[]
\footnotesize
%\centering
\caption{Codebook for Questions}
\label{question-codebook}
\small
%\begin{tabular}{|l|l|l|l|l|l|l|}
\begin{tabular}{ |p{3.5cm}|p{3.5cm}| }
\hline
\textbf{Domain} & \textbf{Question Category}  \\ \hline
  
\multirow{5}{*}{Configuration File} & Store/Version  \\ \cline{2-2}
 & Distribute\\ \cline{2-2}
 & Ignore/Hide \\ \cline{2-2}
 & Exploitability \\ \cline{2-2}
 & Accessibility \\ \hline
 
\multirow{5}{*}{Secrets} & Store/Version  \\ \cline{2-2}
 & Distribute\\ \cline{2-2}
 & Ignore/Hide \\ \cline{2-2}
 & Exploitability \\ \cline{2-2}
 & Accessibility \\ \cline{2-2}
 & Restriction \\ \hline
 
\multirow{5}{*}{Client Side Application} & Store  \\ \cline{2-2}
 & Distribute\\ \cline{2-2}
 & Ignore/Hide \\ \cline{2-2}
 & Accessibility \\ \cline{2-2}
 & Exploitability \\ \hline
 

\multirow{5}{*}{VCS Feature} & History Sanitize  \\ \cline{2-2}
 & Line Level Security\\ \cline{2-2}
 & Encrypt File\\ \cline{2-2}
 & Secrets Copy During Clone\\ \cline{2-2}
 & Ignore Already Committed\\ \hline
 
 
\multirow{5}{*}{Deployment} & Store/Version  \\ \cline{2-2}
 & Distribute\\ \cline{2-2}
 & Ignore/Hide\\ \cline{2-2}
 & Improper Configuration \\ \cline{2-2}
 & Dot File \\ \hline
 
Pre-open Source & Crosscheck \\ \hline

External Secret Management Service & Setup \\ \hline

\multirow{3}{*}{Secureness} & Private Repository \\ \cline{2-2}
& Unpushed Branch\\ \cline{2-2}
& Testing Credentials\\ \hline

\multirow{2}{*}{Others} & Importance \\ \cline{2-2}
& Decision \\ \hline
 
\end{tabular}
\end{table}

==> Tables/SecretsTypes.tex <==
\begin{table}
\begin{center}
\caption{Secrets Counts and Percentages}
\label{secret-types}
\small
\begin{tabular}{|c| c| c|} 
 \hline
 \textbf{Secret} & \textbf{Count} & \textbf{Percentage of Secrets} \\ [0.5ex] 
 \hline\hline
 Database credentials & 117 & 30.6\%\\ 
 \hline
 Secret keys & 81 & 21.2\%\\
 \hline
 API keys & 72 & 18.8\%\\
 \hline
 Passwords & 32 & 8.4\%\\
 \hline
 Tokens & 15 & 3.9\%\\ 
 \hline
 App credentials & 8 & 2.1\%\\ 
 \hline
 Private keys & 7 & 1.8\%\\
 \hline
\end{tabular}
\end{center}
\end{table}

==> Tables/SeparateMappings.tex <==
\begin{table}[]
\footnotesize
\centering
\caption{Configuration File Question to Answer Mappings}
\label{secrets-mapping}
%\begin{tabular}{|l|l|l|l|l|l|}
\begin{tabular}{|p{2.8cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|   }
\hline
 \multirow{2}{*}{\textbf{Answer Categories}} & \multicolumn{5}{c|}{\textbf{Question Categories}} \\ \cline{2-6} 

    & \textbf{Store/Version} & \textbf{Distribute} & \textbf{Ignore/Hide} & \textbf{Accessibility} & \textbf{Exploitability}\\ \hline
   
Rewrite VCS History &  &  & X &  & \\ \cline{1-6} 

 Ignore Sensitive File: & X & X & X &  & \\ \cline{1-6} 
 Configuration File &  &  & X &  & \\ \cline{1-6} 
 .env File &  &  & X &  & \\ \cline{1-6} 
 Secertes in Non-Configruation File &  &  & X &  & \\ \cline{1-6} 
 VCS Feature: &  &  & X &  &\\ \cline{1-6} 
 use of git update-index -- assume unchanged &  &  & X &  &\\ \cline{1-6}
 VCS Flag : git --skip-worktree &  &  & X &  &\\ \cline{1-6}
  Add Files to the Staging Area Explicitly &  &  &  X &  &\\ \cline{1-6} 
   Store Encrypted/Obfuscated Secrets: &X  &  & X &  &\\ \cline{1-6} 
   Bouncy Castle Libs &X  &  &  &  &\\ \cline{1-6} 
   GPG Encryption &X  &  &  &  &\\ \cline{1-6} 
   Protected Configuration? &  &  & X &  &\\ \cline{1-6} 
   Secrets Management in Deployment: & X &  &  & X &\\ \hline %\cline{1-6} 
 Config Transformation &  X&  &  & X  &\\ \cline{1-6}
 Deployment Variables- Heroku Config Variables &  X&  &  &   &\\ \cline{1-6}
 Shared Folder &  X&  &  &   &\\ \cline{1-6}
 Create config file in Deployment  Server &  X&  &  &   &\\ \cline{1-6}
 Run time configuration loading &  &  & X &   &\\ \cline{1-6}
  External Secret Management Service: & X &  &  &  & X\\ \cline{1-6} 
  AWS Parameter Store: & X &  &  &  & \\ \cline{1-6}
  Git-Secrets: & X &  &  &  & \\ \cline{1-6}
  Vault: & X &  &  &  & \\ \cline{1-6}
   Use Environment Variables & X &  & X &  & X\\ \cline{1-6} 
    Remove Original Configuration File & X &  & X &  &\\ \cline{1-6} 
     Use Template Config file & X & X & X &  &\\ \cline{1-6} 
     Move Secrets out of Source Code/Version Control & X & X & X &  & X\\ \cline{1-6} 
     Move Secrets to Configuration File &  & X &  &  & \\ \cline{1-6} 
      Load Externally &  &  & X &  &\\ \cline{1-6}
      Secondary Private Repository & X &  &  &  &\\ \cline{1-6}
      Syntax Error Fix &  &  &  & X &\\ \cline{1-6}
      Exploitable &  &  &  &  &X \\ \cline{1-6}
      Non Exploitable & X &  &  &  & X\\ \hline 
      
\end{tabular}
\end{table}

\begin{table}[]
\footnotesize
\centering
\caption{Secrets Question to Answer Mappings}
\label{my-label}
%\begin{tabular}{|l|l|l|l|l|l|}
\begin{tabular}{|p{2.8cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|   }
\hline
     \multirow{2}{*}{\textbf{Answer Categories}} & \multicolumn{5}{c|}{\textbf{Question Categories}} \\ \cline{2-6} 

    & \textbf{Store/Version} & \textbf{Distribute} & \textbf{Ignore/Hide} & \textbf{Restriction} & \textbf{Exploitability}\\ \hline
    
    
    Revokation and Rotation & X &  & X &  & X\\ \cline{1-6} 
   
Rewrite VCS History &  &  & X &  & X \\ \cline{1-6} 

 Ignore Sensitive File & X &  & X &  & \\ \cline{1-6} 
 VCS Feature &  &  & X &  &\\ \cline{1-6} 
   Store Encrypted/Obfuscated Secrets &X  &  & X &  &\\ \cline{1-6} 
 Deployment Tools &  X&  &  &   &\\ \cline{1-6} 
 Config Transformation &  X&  & X &   &\\ \cline{1-6}
 Deployment Variables &  X&  & X &   &\\ \cline{1-6}
 Shared Folder &  &  & X &   &\\ \cline{1-6}
 Create config file in Deployment Server & X &  &  &   &\\ \cline{1-6}
  External Secret Management Service & X &  & X  &  & \\ \cline{1-6} 
   Use Environment Variables & X &  & X &  & \\ \cline{1-6} 
   Restrict API access and permissions & X &  &  &  &\\ \cline{1-6}
     Use Template Config/Non-Config file & X &  & X &  &\\ \cline{1-6} 
     Move Secrets to Configuration File & X &  & X &  & \\ \cline{1-6}
     Move Secrets out of Source Code/Version Control & X &  & X &  & X\\ \cline{1-6} 
      Load Externally & X & X & X &  &\\ \cline{1-6}
      Secondary Private Repository &  &  & X &  &\\ \cline{1-6}
      Non Exploitable &  &  &  &  & X\\ \hline 
      Exploitable &  &  &  &  & X\\ \hline
      Server Side Implementation
 & X &  & X &  & \\ \hline
\end{tabular}
\end{table}
